Temporally Coherent Embeddings for Self-Supervised Video Representation Learning

This paper presents TCE: Temporally Coherent Embeddings for self-supervised video representation learning. The proposed method exploits inherent structure of unlabeled video data to explicitly enforce temporal coherency in the embedding space, rather than indirectly learning it through ranking or predictive proxy tasks. In the same way that high-level visual information in the world changes smoothly, we believe that nearby frames in learned representations will benefit from demonstrating similar properties. Using this assumption, we train our TCE model to encode videos such that adjacent frames exist close to each other and videos are separated from one another. Using TCE we learn robust representations from large quantities of unlabeled video data. We thoroughly analyse and evaluate our self-supervised learned TCE models on a downstream task of video action recognition using multiple challenging benchmarks (Kinetics400, UCF101, HMDB51). With a simple but effective 2D-CNN backbone and only RGB stream inputs, TCE pre-trained representations outperform all previous selfsupervised 2D-CNN and 3D-CNN pre-trained on UCF101. The code and pre-trained models for this paper can be downloaded at: https://github.com/csiro-robotics/TCE

==> Chapters/OLD-Results.tex <==
\section{Experimental Results} \label{sec:experimentalResults}
\begin{table*}[t]
    \centering
        \caption{Top-1 accuracy performance for action recognition task on UCF101 dataset.  $^{*}$ Network architecture using stack-of-differences for downstream training. $^{**}$ Two networks which do not share weights. $^{+}$ Results reported on train/test split 1 of UCF101.}%\vspace{-0.7cm}}
        \begin{tabular}{llclc}
        \hline 
         Method & Backbone & 2D-CNN & Pre-Training & UCF101 (\%)\\
         \hline
         Motion \& Appearance \cite{wang2019selfsupervised}& C3D & \xmark & Kinetics400  & 61.2 \\
         3DRotNet \cite{jing2018selfsupervised} & 3D ResNet-18 & \xmark & Kinetics400 & 62.9  \\
         3DCubicPuzzles \cite{kim2019self} & 3D ResNet-18 & \xmark & Kinetics400 & 65.8 \\ %63.9$^*$(65.8) \\
         DPC \cite{han2019video} & 3D ResNet-18 & \xmark & Kinetics400 & 68.2\\
         DPC \cite{han2019video} & 3D ResNet-34 & \xmark & Kinetics400 & \textbf{75.7} \\
         \hline
         Shuffle and Learn \cite{misra2016shuffle}$^+$ & AlexNet & \cmark & UCF101 & 50.9\\
         VideoGAN \cite{vondrick2016generating} & C3D & \xmark & UCF101 & 52.1 \\
         Arrow of time \cite{wei2018learning}& AlexNet & \cmark & UCF101 & 55.3 \\
         OPN \cite{fernando2017self} & AlexNet & \cmark & UCF101 & 56.3\\
         CMC \cite{tian2019contrastive} & CaffeNet $\times 2^{**}$ & \cmark & UCF101 & 59.1 \\
         Motion \& Appearance \cite{wang2019selfsupervised}& C3D & \xmark & UCF101 & 58.8  \\
         O3N \cite{fernando2017self} & AlexNet$^{*}$ & \cmark & UCF101 & 60.3 \\
         DPC \cite{han2019video} & 3D ResNet-18 & \xmark & UCF101 & 60.6 \\
         Skip-Clip \cite{el2019skip}$^+$ & 3D ResNet-18 & \xmark & UCF101  & 64.4\\ %59.5$^*$(64.4) \\
         Video Clip Ordering \cite{xu2019self}$^+$ & R3D & \xmark & UCF101 & 64.9 \\
         \hline 
         %Ours & AlexNet & UCF101 & \\
         \textbf{\textit{TCE} (Ours)$^+$} & ResNet-50$^{*}$ & \cmark & UCF101 & \textbf{67.01}\\
         \hline 
        \end{tabular}
    
    \label{tab:soa_table}
\end{table*}

In this section we evaluate the performance of our proposed method in a number of ways. We trained a classification network on an action recognition task using the self-supervised learned representation. We investigate the effect that training with multiple negatives has on results, in addition to the method of network initialization, and the effects of enforcing higher order temporal coherency. We also directly evaluate the features that our method produces against those from other training methods including ImageNet pretraining.  The code and pre-trained models used in this paper can be downloaded at \href{https://github.com/csiro-robotics/TCE}{https://github.com/csiro-robotics/TCE}.
%
\subsection{Dataset}
\textit{TCE} is a generalised method of learning robust representations of video data. Here we focus on the task of video action recognition.  Specifically, we train and evaluate \textit{TCE} on the UCF101 dataset~\cite{soomro2012ucf101}. Containing 101 human action classes and 13,000 videos, UCF101 is a common benchmark dataset for both action recognition as well as many self-supervised approaches. Three different train/test splits were released with the data. Aligning with self-supervised methods ~\cite{xu2019self,misra2016shuffle} and~\cite{el2019skip}, we train and evaluate on the first train/test split. 

\subsection{Self-Supervised Training}
We train an embedding function on the UCF101 dataset without labels to learn robust video representations. The network architecture on which we train is ResNet-50 \cite{he2016deep}. We initialize the network with random weights and train for a total of 9 epochs with 4 Tesla-V100 GPUs. Training is completed using a stochastic gradient descent optimiser and batch size of 100. Initially a learning rate of 0.03 is used and reduced by a factor of 10 after 5 epochs. Positive examples are taken by sampling two adjacent video frames from the dataset, and each frame in the dataset is used as a positive example once per epoch. 
%
During training, frames are resized so that the shortest side is 256 pixels while preserving image scale, and are then randomly cropped to a $224\times224$ window. Random horizontal flipping is also employed.

$N_1 = 8192 $ negative samples used in optimizing first order coherency are drawn from randomly selected videos in the dataset, excluding the video from which positive examples were drawn. Our rationale behind this sampling regime is that by sampling from videos other than the positive embeddings, we ensure our negatives are significantly different in appearance. 
%
For higher order coherency experiments, $N_2$ = 100 negative examples are sampled from within the same video as the positive examples are drawn. $N_2$ is significantly smaller than $N_1$ as the number of frames available in a single video is significantly smaller than those in the rest of the dataset.
    

Inspired by Wu~\etal~\cite{wu2018unsupervised}, we maintain a memory bank to store embeddings for each frame in the dataset to efficiently retrieve noisy samples without re-computing their embeddings. The memory bank is dynamically updated with the new embeddings on every forward pass of the network.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Action Recognition}\label{subsec:datasets}


\subsubsection{Training}
\label{subsec:results}
%
    We benchmark the quality of our learned embedding function by finetuning our network for action recognition on the UCF101 \cite{soomro2012ucf101} dataset, which contains in excess of 13,000 videos of 101 action classes. Following \cite{misra2016shuffle,el2019skip,xu2019self} we perform experiments and report on the first test/train split of the dataset.
    
    During training, we replace the final fully connected layer of our pretrained network with another fully-connected layer of 101 nodes, using the ReLu activation function. 
    %
    We employ the stack-of-differences video-clip encoder introduced by \cite{fernando2017self}. Six neighbouring frames are taken from the video to produce an input with size ${224}\times{224}\times15$ by resizing each image to $224 \times 224$ pixels and taking the differences between the five neighbouring pairs of frames. The convolutional layers of our pretrained network are duplicated five times in order to allow the 15-channel input to be fed through the network. 
    
    During evaluation, nineteen evenly-spaced blocks of six frames are taken from each video. Softmax outputs on each block of frames are averaged, and the highest average value is the classification output for the video. We report results for the highest scoring epoch during training for all our experiments.
%
    The network is trained using 4 Tesla-V100 GPUs and stochastic gradient descent for 600 epochs with a learning rate of 0.05 that is decayed by a factor of 10 after 350 epochs. 
    
%

%\vspace{-4mm}
\subsubsection{Comparison to State-of-the-Art}
\label{subsec:SOA}
The results of our training method are compared against other state-of-the-art results in Table \ref{tab:soa_table}. We achieve higher Top-1 classification accuracy with pretraining on the UCF101 dataset than any other approach in the literature which trains on the same dataset, as far as we are aware. Notably this is irrespective of network architecture and our approach implemented on ResNet50 outperforms Video Clip Ordering \cite{xu2019self} -- which uses 3D ResNet18 as the network backbone -- by 3.8\% despite being implemented on a 2D convolutional network.
  
Our approach also surpasses the vast majority of the those pre-trained on the Kinetics400 dataset despite using a significantly smaller dataset for pre-training. The only approach in the literature which surpasses our result is Dense Predictive Coding (DPC) \cite{han2019video} which is both trained on the Kinetics400 \cite{carreira2017quo} - which contains 306K video clips, as opposed to only 13K for UCF - and employs the extremely high capacity 3D ResNet-34 network architecture.  Notably, DPC's network took six weeks to train \cite{han2019video}, while our approach completed pre-training and fine-tuning on action recognition within four days.  We plan to explore use of Kinetics400 in future work to demonstrate the scalability of our method to larger datasets.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of Results}\label{subsec:pretraining}
    In this section we detail experiments to analyse the performance of \textit{TCE}. We compare our results to random network initialization and ImageNet pretraining in order to gauge how our choice of network architecture and loss function impacts the performance of the downstream action-recognition task, and also investigate how changing the number of negatives sampled affects performance. Finally, we investigate how higher order coherency objectives affect the results achieved.
    
    %\vspace{-4mm}
    \subsubsection{Comparison to Random Initialization} Table \ref{tab:init_methods} details the performance achieved by our network on the action recognition task when trained from randomly initialized weights, ImageNet pretrained weights, and our self-supervised representation,\textit{TCE}.
    
    %\vspace{-5mm}    
    \begin{table}[h]
        \caption{Top-1 accuracy performance for action recognition task on UCF101 dataset for different initialization methods of our network.}
        \begin{tabular}{lc}
            \hline 
            \textbf{Initialization} \hspace{10mm} & \hspace{5mm} \textbf{UCF101} \hspace{5mm} \\
            \hline \hline 
            Random & 59.82 \\
            \hline
            ImageNet &  77.69\\
            \hline
            \textit{TCE} (Ours) & 67.01  \\
            \hline 
        \end{tabular}
        \label{tab:init_methods}
    \end{table}
    %\vspace{-3mm}
    
    We report a 14.9\% improvement over training from random weights and achieve 88.5\% of the ImageNet pretraining baseline.
    %
    This significant improvement demonstrates that our embedding space learns features which generalise well to the task of action recognition and further validates \textit{TCE} against the standard approach of full supervision.
%
    Notably, the combination of ResNet50 and stack-of-differences in the downstream task achieves 59.82\% accuracy after training with randomly initialized weights, well above results on AlexNet quoted in \cite{fernando2017self,misra2016shuffle,wei2018learning}.
  
    

\begin{figure}[t]
    \centering
    \includegraphics[width=60mm]{figures/negatives.png}
    \caption{Top-1 Accuracy on UCF101 action recognition task versus the number of negative examples used during training.}
\label{fig:negative_graph}
 \end{figure}


    \noindent \textbf{Investigating the Effects of Negative Samples} We also investigated how the number of negative examples sampled when calculating first-order cross-entropy loss affect performance on the action recognition downstream task.
    %
    Fig. \ref{fig:negative_graph} illustrates the relationship between the number of negative examples sampled, and the Top-1 classification accuracy on the action recognition classification task.
    %
    We found we achieved our highest accuracy using 8192 negatives, which we've used to calculate our final result.
    
    


    
    
    
    \noindent \textbf{Investigating the Effects of High-Order Coherency Objectives} We investigate the effect of implementing a higher-order loss term to \textit{TCE}, with results presented in Table \ref{tab:ablations}. The First + Second Order result is trained on a total loss which is the sum of the first-order coherency loss introduced in Equation \ref{eq:cross-entropy} with the second-order loss introduced in Equation \ref{eq:SecondOrder}.
    
    %\vspace{-5mm}
    \begin{table}[h]
        \centering
        \caption{Action recognition performance on UCF101 when training \textit{TCE} with and without enforcing a second-order coherency.}
        \begin{tabular}{lc}
            \hline 
             \textbf{Method} \hspace{10mm} & \hspace{5mm}\textbf{UCF101}\hspace{5mm} \\
             \hline \hline 
             First Order Only &  67.46\\
             \hline
             First + Second Order & 66.35\\
             %\hline 
             %Ours + Rotation & \\
             \hline 
        \end{tabular}
        \label{tab:ablations}
    \end{table}
    %\vspace{-6mm}
    
    In both training cases, we pretrain on UCF101 with $N_1=4096$ and $N_2 = 100$ negatives when calculating first and second-order loss terms respectively. $N_2$ is lower than $N_1$ as the number of frames available in a single video is significantly smaller than those in the rest of the dataset.
    
    We found that implementing a higher order coherency term to the loss function resulted in diminished downstream performance for action recognition, compared to simply training with first-order loss. We believe that this is because the within-video negative examples are too similar to the positive examples and act as noise when learning, hindering the overall performance. Other methods which leverage negative examples from within-video introduce a temporal buffer to ensure that negative examples are temporally distant to the positive examples and so are easier for the network to distinguish during training. We have included a similar study in the supplementary materials.




==> Chapters/comments.tex <==
% ========= Author Comments

Comments to author (Associate Editor)
=====================================

Reviewers are positive on this paper. AC also agrees
that this work is interesting and deserved to be published
on ICPR. The reviewers did raise some valuable concerns
that should be addressed in the final camera-ready version
of the paper. The authors are encouraged to make the
necessary changes.

Important: please include recent works on self-supervised
video representation learning.
[1] Self-supervised video representation learning with
space-time cubic puzzles. AAAI 2019
[2]Geometry guided convolutional neural networks for
self-supervised video representation learning. CVPR 2018



----------------------------------------
Comments on Supplementary material:

[None found]

Changes to make:
 - Insert references
 - 

% ========= Reviewer 1

Reviewer 1 of ICPR 2020 submission 2462

Comments to the author
======================

Fig.1 is not appropriate to be exposed as a teaser image in
page 1. To me it doesn't give a high level overview of the
paper contribution, it's more like visualizing the outcome
of an experiment.

I am not fully aware of the sota on the specific topic so i
am not best at judging the novelty in the method. The
approach however seems to be based on reliable assumption
(temporal consistency) and reasonable motivation.

Frame-based models for video (2D cnn feature extraction +
late temporal aggregation) are becoming less attractive
and, unless justified by application constraints, it would
be more interesting now to investigate lightweight
spatio-temporal backbone CNNs also in the context of
self-supervised learning. In this sense i see my interest
in the paper is limited.

The assumption "We consider a pair of temporally
neighbouring frames from one video as positive examples,
and consider all frames from other videos to be negative
examples." may be flawed in a video classification task.
There might well be different videos with close appearance
in a video classification dataset. Does your method handle
the case where a same video clip is copied twice into a
dataset? The negative video sampling appears to me a key
aspect but it is not taken into consideration properly.

Changes to make:
 - Clarify how our negative mining helps deal with the hard examples DONE

% ========= Reviewer 2

Reviewer 2 of ICPR 2020 submission 2462

Comments to the author
======================

The paper presents a self-supervised representation
learning of spatio-temporal features from videos. The code
and pre-trained models are available for download. The
accuracy is not very impressive but should increase if more
features (e.g. audio) are considered.

Changes to make: 
 - None

% ========= Reviewer 3

Reviewer 3 of ICPR 2020 submission 2462

Comments to the author
======================

For the experimental part, the three ablation experiments
are only tested on UCF101, including the comparison of
first-order loss and second-order loss, which is slightly
limited. In the data set size comparison section, the
control experiments between HMDB51 and UCF101, HMDB51 and
K400 are missing. In addition, the test results of
2D-ResNet50 on UCF101 in Table IV and Table V are
inconsistent, the former is 72.14 and the latter is 71.2.
For the writing part, first of all, there is no background
introduction in the abstract part, in which the model is
introduced directly. Second, the spelling of British and
American words is mixed, so a unified format is
recommended. Third, there are spelling and grammatical
errors in some sentences, as well as omission of
punctuation. Fourth, the result analysis part is too long,
and it is recommended to be  generalized. Fifth, the
conclusion section is too detailed. It is strongly
recommended to summarize the three paragraphs into one
paragraph.

Changes to make: 
 - Mix of british and American spelling - fix DONE
 - Proof read spelling and grammar DONE
 - 



